A Pilot Study on Visually Stimulated Cognitive Tasks for EEG-Based Dementia Recognition

In the status quo, dementia is yet to be cured. Precise diagnosis prior to the onset of the symptoms can prevent the rapid progression of the emerging cognitive impairment. Recent progress has shown that Electroencephalography (EEG) is the promising and cost-effective test to facilitate the detection of neurocognitive disorders. However, most of the existing works have been using only resting-state EEG. The efficiencies of EEG signals from various cognitive tasks, for dementia classification, have yet to be thoroughly investigated. In this study, we designed four cognitive tasks that engage different cognitive performances: attention, working memory, and executive function. We investigated these tasks by using statistical analysis on both time and frequency domains of EEG signals from three classes of human subjects: Dementia (DEM), Mild Cognitive Impairment (MCI), and Normal Control (NC). We also further evaluated the classification performances of two features extraction methods: Principal Component Analysis (PCA) and Filter Bank Common Spatial Pattern (FBCSP). We found that the working memory related tasks yielded good performances for dementia recognition in both cases using PCA and FBCSP. Moreover, FBCSP with features combination from four tasks revealed the best sensitivity of 0.87 and the specificity of 0.80. To our best knowledge, this is the first work that concurrently investigated several cognitive tasks for dementia recognition using both statistical analysis and classification scores. Our results yielded essential information to design and aid in conducting further experimental tasks to early diagnose dementia patients.

==> 5_Conclusion.tex <==
% In this paper, we present four cognitive tasks as a visual stimulation for classifying cognitively impaired patients into three groups with their brain signals, EEG.
% In order to differentiate, analyses were performed on two types of feature domains: frequency and time.
% For the frequency-domain analysis, the data were pre-processed and transformed into frequency-based features, then, relative power were calculated. The distinctive features were selected with FBCSP algorithm and later classified with the Support Vector Machine (SVM).
% For the time-domain analysis, the data were pre-processed and analyzed on the time features extracted from Event-Related Potential based on their time features.
% The classification-based algorithm, SVM, was adopted in order to classify subjects into their respective classes (NC, MCI, DEM).
% The performance of these analysis methods on four cognitive tasks were compared.
% The classification results revealed that the best performance was achieved individually by the mental imagery task in frequency-domain analysis and the symbol recognition task in the time-domain analysis. 
% Lastly, the better discrimination between normal controls and dementia patients from 4-task combinations proposed an alternative way to improve the machine learning classification using the multiple experimental tasks integration.


In this paper, we present four visual stimulation tasks for detection of dementia and classifying subjects based on their brain signals for three groups: (i) Normal Control (NC), (ii) Mild Cognitive Impairment (MCI), and (iii) Dementia (DEM). Unlike previous works that focus on Alzheimer's Disease, we generalize our experiments to Dementia.
To conduct this classification, we have analyzed the EEG signals over two types of features.
For the time-frequency analysis, the data was pre-processed and transformed into frequency-based features, and then the relative power was calculated. The discriminative features were selected with the FBCSP algorithm and used as input of the Support Vector Machine (SVM) to classify the patients into their respective classes (NC, MCI, DEM). Our work is the first study that attempts to use the FBCSP algorithm to extract EEG features for dementia recognition. 
For the time analysis, the data was pre-processed and transformed into Event-Related Potential. Then, we extracted the distinctive features using the Principal Components Analysis (PCA) and used them as the input of an SVM to classify the subjects.
The classification results revealed that the best performance was achieved by the Mental Imagery task in time-frequency analysis and the Symbol Recognition task in the time-domain analysis. However, combining the 4-tasks yielded the highest performance model to discriminate the normal control and dementia classes. This result suggests that we should base our classification models on a combination of tasks rather than just relying solely on one task.
The suitable number of trials that yields the best accuracy in classifying cognitive decline with the proposed tasks, the performance is best with less than 20 trials (17 trials+ 3 testing trials). 
